Schema Augmentation for Zero-Shot Domain Adaptation in Dialogue State Tracking

Zero-shot domain adaptation for dialogue state tracking (DST) remains a challenging problem in task-oriented dialogue (TOD) systems, where models must generalize to target domains unseen at training time. Current large language model approaches for zero-shot domain adaptation rely on prompting to introduce knowledge pertaining to the target domains. However, their efficacy strongly depends on prompt engineering, as well as the zero-shot ability of the underlying language model. In this work, we devise a novel data augmentation approach, Schema Augmentation, that improves the zero-shot domain adaptation of language models through fine-tuning. Schema Augmentation is a simple but effective technique that enhances generalization by introducing variations of slot names within the schema provided in the prompt. Experiments on MultiWOZ and SpokenWOZ showed that the proposed approach resulted in a substantial improvement over the baseline, in some experiments achieving over a twofold accuracy gain over unseen domains while maintaining equal or superior performance over all domains.

==> updated_sections/ourapproach.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% CHRIS's VERSION BELOW %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We consider textual inputs of the following form:
% \begin{align}
%     x = \text{concat}(c, q)
% \end{align}
% where $c$ is context and $q$ is the query. Context refers to any information about the task or domain which potentially does not vary from sample to sample, while the query is the part of the input which varies in every sample. In our case, instructions and schema constitute $c$, while the dialogue comprises $q$. 

% \subsection{Schema Augmentation}
% The primary problem we seek to address, domain adaptation, stems from the fact that the target domains are not present in the training data. To alleviate this, we propose Schema Augmentation, a method that utilizes data augmentation to improve domain generalization with fine-tuning while requiring no training samples from the target domain. We introduce an augmenting function $g(c)$ which alters the context in some way. Data augmentation is typically used to improve robustness to unseen data by altering the entire input. Because our goal is to generalize across domains, we propose to perform augmentation on the context $c$, which provides domain information, rather than the full input. We then train on the augmented dataset:
% \begin{gather}
%     x = \text{concat}(c, q) \\
%     x' = \text{concat}(g(c), q) \label{eqn:xprime} \\
%     \mathcal{X}' = \{(x',y)\}
% \end{gather}
% The augmented training set thus becomes
% \begin{align}
%     \mathcal{X}_\text{train}^{\text{aug}} = \mathcal{X}_\text{train} \cup \mathcal{X}'_\text{train}
% \end{align}
% We experiment with various forms of $g(c)$ to determine the most effective method for this problem.


% We experiment with two forms of $\alpha(c)$ (Equation \ref{eqn:xprime}). In the first form, we replace slot names with semantically equivalent alternatives using synonymous terms. For example, \texttt{restaurant-area} $\rightarrow$ \texttt{eatery-location}. The synonyms were provided by prompting Gemini \cite{team2023gemini} to create a list of synonyms for each domain and slot name, given a description of the task and an example for context. The model was asked to order the synonyms by relevance. We experimented with two alterations of this form: in the first, we used top-1 synonyms replacement, where each domain and slot name was always replaced by the top (most relevant) synonym (denoted top-1). Thus only two forms of each name appear in the training data. In the second alteration, we randomly chose a synonym from the list for every sample independently (denoted rng). Thus the same slot can have several different forms represented in one dialogue across multiple turns.

% In the second form of $g(c)$, we replace each slot name with an encoded version with no semantic relationship with the original name, e.g. \texttt{restaurant-area} $\rightarrow$ \texttt{domain6-slot2}. In this case, the model must make use of the rest of the context (slot description and possible values) to discern the correct slots to generate in the response. This encourages the model to attend to tokens in the descriptions and possible values more strongly, which provide crucial information for the target domains at test time.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% ROSHAN's VERSION BELOW %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Domain adaptation can be addressed by utilizing examples of data from the target domains, either in fine-tuning \cite{dingliwal2021few,zeng2021domain}, or as few-shot examples during inference \cite{yang2023dual,chen2023stabilized,rastogi2019scaling,hu2022context}. However, obtaining reliably annotated data for unseen domains is not possible in many practical situations. Therefore, we propose to augment existing training data with modified versions of the same that are designed to be similar to data from unseen test domains. 

% To design the augmentation transform, we note that examples from a new domain differ from examples in existing domains in two ways -- the labeling schema, and the user-assistant interaction. We hypothesize that large language models are likely robust to variations in user-assistant interactions due to the large amounts of text they are pre-trained on, and focus on differences in schema. 

% We introduce \emph{Schema Augmentation}, a method that generates augmented training data by modifying the domain names and slot names. The key principle underlying schema augmentation is that we can create a myriad of schemas during training and associate them with user-assistant interactions from training domains, and the resulting model should be more robust to schema changes, i.e., domain shifts during inference. 

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{images/gtod_figure1.png}
    \caption{Examples of domain and slot replacements for both Schema Augmentation types: SSA (blue box) and ESA (green box). A full example of augmented prompts can be found in Appendix }
    \label{fig:example}
\end{figure}



Domain adaptation is often addressed by leveraging target domain data for fine-tuning \cite{dingliwal2021few,zeng2021domain} or as few-shot examples during inference \cite{yang2023dual,chen2023stabilized,rastogi2019scaling,hu2022context}. However, reliably annotated data for unseen domains is often unavailable. To address this, we propose to achieve zero-shot adaptation through data augmentation. New domains differ from existing ones in their labeling schema and dialogues. Large language models (LLMs), pre-trained on vast amounts of natural language, are likely robust to variations in dialogue, so we focus on differences in schema.

Our method, \emph{Schema Augmentation}, generates augmented data by altering domain and slot names to enhance the model’s robustness to schema changes. We introduce two types of Schema Augmentation. First, in \textbf{Synonym Schema Augmentation (SSA)}, we replace domain and slot names with synonyms. Second, in \textbf{Encoding Schema Augmentation (ESA)}, we replace domains and slots with non-semantic codes, requiring the model to rely on slot descriptions and possible values to predict the dialogue state accurately. Figure \ref{fig:example} shows examples of each method.

For both types of augmentation, we experiment with two variations: single and multi. In single-SSA and single-ESA, we use a static synonym or code replacement for each domain and slot. In multi-SSA and multi-ESA, we randomly select the replacement for each sample from a pre-determined list. Gemini \cite{team2023gemini} provides the synonym lists, while we create encodings by appending integers to ‘domain’ or ‘slot.’ In multi-ESA, we ensure non-overlapping encodings for each domain and slot by using disjoint ranges of integers. The replacements used in both cases are provided in Appendix \ref{sec:appendix}.
